DocSum: Domain-Adaptive Pre-training for Document Abstractive Summarization

Abstractive summarization has made significant strides in condensing and rephrasing large volumes of text into coherent summaries. However, summarizing administrative documents presents unique challenges due to domain-specific terminology, OCR-generated errors, and the scarcity of annotated datasets for model fine-tuning. Existing models often struggle to adapt to the intricate structure and specialized content of such documents. To address these limitations, we introduce DocSum, a domain-adaptive abstractive summarization framework tailored for administrative documents. Leveraging pre-training on OCR-transcribed text and fine-tuning with an innovative integration of question-answer pairs, DocSum enhances summary accuracy and relevance. This approach tackles the complexities inherent in administrative content, ensuring outputs that align with real-world business needs. To evaluate its capabilities, we define a novel downstream task setting-Document Abstractive Summarization-which reflects the practical requirements of business and organizational settings. Comprehensive experiments demonstrate DocSum's effectiveness in producing high-quality summaries, showcasing its potential to improve decision-making and operational workflows across the public and private sectors.

==> sections/03_datasets.tex <==
\subsection{Overview}
Our study uses the Administrative Document Images from the IIT-CDIP collection\footnote{\url{https://data.nist.gov/pdr/lps/ark:/88434/mds2-2531}} and the RVL-CDIP dataset\footnote{\url{https://adamharley.com/rvl-cdip/}}. These administrative documents were made publicly available as part of legal proceedings and settlements against several American tobacco and cigarette companies and organizations in the 1990s. As a result, the corpus of two datasets are related to the American tobacco industry and were created during the 1980s and 1990s. While these datasets have been widely used for NLP tasks such as text recognition, classification, layout analysis, etc., this is the first study to apply them to text summarization.  

Our model is pre-trained on the IIT-CDIP datasets and fine-tuned for specific tasks using the RLV-CDIP dataset.

\noindent \textbf{Pre-training dataset.} The IIT-CDIP database includes page of scanned documents. Each page was stored as grayscale TIFF images and was handle-labeled into a variety of categories, including telex, speech, note, email, promotion, and many others. In this dataset, one page can be assigned multiple classes, as documents often contain different types of content. Moreover, each document has corresponding text extracted by 90s-era OCR and metadata stored in XML files.

\noindent\textbf{Downstream dataset.} Similar to the previous dataset, RVL-CDIP has the same structure. However, there are only 16 document classes: letter, memo, email, file folder, form, handwritten, invoice, advertisement, budget, news article, resume, presentation, publication, questionnaire, report, and specification. Each page belongs to a single category. The public TesseractOCR library was used for text generation. 

\subsection{Data Pre-processing}
\noindent \textbf{Data Filtering.} 
All the duplicated or empty content was removed to maintain data quality. For the RLV-CDIP dataset, we also filtered out documents with fewer than 100 words to ensure that documents are not too short to summarize.

\noindent \textbf{Subset Selection for Experiments.} 
In order to reduce processing time and resource usage, we only work with subsets of both datasets: 100,000 and 40,000 documents of IIT-CDIP and RVL-CDIP, respectively.

\noindent \textbf{Label cleanup.}
The categories of an image in the IIT-CDIP dataset are pretty chaotic because manual annotations cause one class to have different names, such as \textit{tele, telex, tlx}, etc. Consequently, models potentially confuse and treat documents in the same class as different entities. Therefore, we need to uniformize class names across the entire dataset to ensure the quality for the data. 

